Illuminating the Space of Dungeon Maps, Locked-door Missions and Enemy Placement Through MAP-Elites

Procedural Content Generation (PCG) methods are valuable tools to speed up the game development process. Moreover, PCG may also present in games as features, such as the procedural dungeon generation (PDG) in Moonlighter (Digital Sun, 2018). This paper introduces an extended version of an evolutionary dungeon generator by incorporating a MAP-Elites population. Our dungeon levels are discretized with rooms that may have locked-door missions and enemies within them. We encoded the dungeons through a tree structure to ensure the feasibility of missions. We performed computational and user feedback experiments to evaluate our PDG approach. They show that our approach accurately converges almost the whole MAP-Elite population for most executions. Finally, players' feedback indicates that they enjoyed the generated levels, and they could not indicate an algorithm as a level generator.

==> Breno FDG2022/images/methodology/map-representation.tex <==
\begin{figure}[!t]
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.7}]
    % Node style
    \tikzstyle{node} = [draw, minimum size=1cm]

    % 
    \node[node] (l1c1) at (0,0) { };
    \node[node] (l1c2) [right = 0.15cm of l1c1] { };
    \node[node] (l1c3) [right = 0.15cm of l1c2] { };
    \node[node] (l1c4) [right = 0.15cm of l1c3] { };
    \node[node] (l1c5) [right = 0.15cm of l1c4] { };
    % 
    \node[node] (l2c1) [below = 0.15cm of l1c1] { };
    \node[node, thick, red!70!black] (l2c2) [right = 0.15cm of l2c1] { };
    \node[node] (l2c3) [right = 0.15cm of l2c2] { };
    \node[node] (l2c4) [right = 0.15cm of l2c3] { };
    \node[node] (l2c5) [right = 0.15cm of l2c4] { };
    % 
    \node[node] (l3c1) [below = 0.15cm of l2c1] { };
    \node[node] (l3c2) [right = 0.15cm of l3c1] { };
    \node[node] (l3c3) [right = 0.15cm of l3c2] { };
    \node[node] (l3c4) [right = 0.15cm of l3c3] { };
    \node[node] (l3c5) [right = 0.15cm of l3c4] { };
    % 
    \node[node] (l4c1) [below = 0.15cm of l3c1] { };
    \node[node] (l4c2) [right = 0.15cm of l4c1] { };
    \node[node] (l4c3) [right = 0.15cm of l4c2] { };
    \node[node, thick, blue!70!black] (l4c4) [right = 0.15cm of l4c3] { };
    \node[node] (l4c5) [right = 0.15cm of l4c4] { };
    % 
    \node[node] (l5c1) [below = 0.15cm of l4c1] { };
    \node[node] (l5c2) [right = 0.15cm of l5c1] { };
    \node[node] (l5c3) [right = 0.15cm of l5c2] { };
    \node[node] (l5c4) [right = 0.15cm of l5c3] { };
    \node[node] (l5c5) [right = 0.15cm of l5c4] { };
    
    % Axis
    \node (ax) [below left = 0.15cm of l5c1] { };
    \node (ax_y1) [above left = 0.15cm of l1c1] { };
    \node (ax_y2) [below right = 0.15cm of l5c5] { };
    
    %
    \draw[->] (ax.center) -- (ax_y1.center);
    \path (ax) -- node [rotate=90,below left=-0.45cm and 1.5cm] {\textbf{Leniency}} (ax_y1);
    \node (le1) [left = 0.3cm of l1c1] {$(0.5,0.6)$};
    \node[thick, red!70!black] (le2) [left = 0.3cm of l2c1] {$(0.4,0.5)$};
    \node (le3) [left = 0.3cm of l3c1] {$(0.3,0.4)$};
    \node[thick, blue!70!black] (le4) [left = 0.3cm of l4c1] {$(0.2,0.3)$};
    \node (le5) [left = 0.3cm of l5c1] {$(0.1,0.2)$};
    
    %
    \draw[->] (ax.center) -- (ax_y2.center);
    \path (ax) -- node [below right=0.5cm and -1cm] {\textbf{Exploration Coefficient}} (ax_y2);
    \node (ce1) [below = 0.3cm of l5c1] {$(0.5,0.6)$};
    \node[thick, red!70!black] (ce2) [below = 0.3cm of l5c2] {$(0.6,0.7)$};
    \node (ce3) [below = 0.3cm of l5c3] {$(0.7,0.8)$};
    \node[thick, blue!70!black] (ce4) [below = 0.3cm of l5c4] {$(0.8,0.9)$};
    \node (ce5) [below = 0.3cm of l5c5] {$(0.9,1.0)$};
    
    % 
    \draw[dashed, thick, red!70!black] (le2) -- (l2c2);
    \draw[dashed, thick, red!70!black] (ce2) -- (l2c2);
    
    \draw[dashed, thick, blue!70!black] (le4) -- (l4c4);
    \draw[dashed, thick, blue!70!black] (ce4) -- (l4c4);
    \end{tikzpicture}

    \caption{The map of MAP-Elites population. The red cell represents a dungeon with leniency between 0.4 and 0.5 and an exploration coefficient between 0.6 and 0.7. The blue cell represents a dungeon with leniency between 0.2 and 0.3 and an exploration coefficient between 0.8 and 0.9. Thus, the blue level has more reference rooms further to each other than the red one, and it also has more rooms with enemies.}
    \label{fig:map-representation}
\end{figure}

==> Breno FDG2022/images/methodology/tree-representation.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}[t]{\columnwidth}
        \centering
        \begin{tikzpicture}[every node/.style={scale=0.7}]
        % Node style
        \tikzstyle{node} = [draw, circle, minimum size=0.7cm]

        % Depth 0, root
        \node[node, thick] (n1) at (0,0) {$S$};
    
        % Depth 1
        \node[node, thick, yellow!70!black] (n2) [below = 0.3cm of n1] {$D$};
        \node[node, thick, blue!70!black] (n3) [right = 1.7cm of n2] {$L$};
        \node[node, thick, red!70!black] (n4) [left = 1.7cm of n2] {$R$};
    
        % Depth 2
        \node[node, thick, yellow!70!black] (n5) [below = 0.3cm of n4] {$D$};
        \node[node, thick, blue!70!black] (n6) [right = 0.3cm of n5] {$L$};
        \node[node, thick, red!70!black] (n7) [left = 0.3cm of n5] {$R_1$};
        
        \node[node] (n8) [below = 0.3cm of n2] {$D$};
        
        \node[node, opacity=0] (an3) [below = 0.3cm of n3] {$0$};
        \node[node] (n9) [left = 0.3cm of an3] {$R_2$};
        
        % Depth 3
        \node[node, opacity=0] (an8) [below = 0.3cm of n8] {$0$};
        \node[node] (n10) [left = 0.3cm of an8] {$R$};
        
        % Depth 3
        \node[node, opacity=0] (an9) [below = 0.3cm of n10] {$0$};
        \node[node] (n11) [right = 0.3cm of an9] {$L$};
        
        % Connect nodes
        \path[draw] (n1) -- (n2);
        \path[draw, dashed] (n1) -- (n3)
            node[pos=0.5,fill=white,inner sep=1]{1};
        \path[draw] (n1) -- (n4);
        
        \path[draw] (n4) -- (n5);
        \path[draw] (n4) -- (n6);
        \path[draw] (n4) -- (n7);
        
        \path[draw] (n2) -- (n8);
        \path[draw] (n8) -- (n10);
        \path[draw, dashed] (n10) -- (n11)
            node[pos=0.5,fill=white,inner sep=1]{2};
        
        \path[draw] (n3) -- (n9);
        \end{tikzpicture}
        \subcaption{Dungeon level genotype.}
        \label{fig:tree-encoding}
    \end{subfigure}
    
    \begin{subfigure}[t]{\columnwidth}
        \centering
        \begin{tikzpicture}[every node/.style={scale=0.7}]
        % Node style
        \tikzstyle{room} = [draw, minimum size=0.7cm]
        \tikzstyle{corridor} = [draw, minimum size=0.7cm, dotted]
        \tikzstyle{empty_room} = [draw, minimum size=0.7cm, dashed]
        \tikzstyle{none} = [draw, minimum size=0.7cm, opacity=0]
        \tikzstyle{coordinate} = [minimum size=0.7cm]
        
        \node[coordinate]
            (l0n0) [] { };
        \node[coordinate]
            (l0n1) [right = 0cm of l0n0] {$-4$};
        \node[coordinate]
            (l0n2) [right = 0cm of l0n1] {$-3$};
        \node[coordinate]
            (l0n3) [right = 0cm of l0n2] {$-2$};
        \node[coordinate]
            (l0n4) [right = 0cm of l0n3] {$-1$};
        \node[coordinate]
            (l0n5) [right = 0cm of l0n4] {$0$};
        \node[coordinate]
            (l0n6) [right = 0cm of l0n5] {$1$};
        \node[coordinate]
            (l0n7) [right = 0cm of l0n6] {$2$};
        %
        \node[coordinate]
            (l1n0) [below = 0cm of l0n0] {$-2$};
        \node[empty_room]
            (l1n1) [right = 0cm of l1n0] { };
        \node[corridor]
            (l1n2) [right = 0cm of l1n1] { };
        \node[room, thick, red!70!black]
            (l1n3) [right = 0cm of l1n2] {$R_1$};
        \node[corridor]
            (l1n4) [right = 0cm of l1n3] { };
        \node[empty_room]
            (l1n5) [right = 0cm of l1n4] { };
        \node[corridor]
            (l1n6) [right = 0cm of l1n5] { };
        \node[empty_room]
            (l1n7) [right = 0cm of l1n6] { };
        %
        \node[coordinate]
            (l2n0) [below = 0cm of l1n0] {$-1$};
        \node[corridor]
            (l2n1) [right = 0cm of l2n0] { };
        \node[none]
            (l2n2) [right = 0cm of l2n1] { };
        \node[corridor]
            (l2n3) [right = 0cm of l2n2] { };
        \node[none]
            (l2n4) [right = 0cm of l2n3] { };
        \node[corridor]
            (l2n5) [right = 0cm of l2n4] { };
        \node[none]
            (l2n6) [right = 0cm of l2n5] { };
        \node[corridor]
            (l2n7) [right = 0cm of l2n6] { };
        %
        \node[coordinate]
            (l3n0) [below = 0cm of l2n0] {$0$};
        \node[room, thick, yellow!70!black]
            (l3n1) [right = 0cm of l3n0] {$D$};
        \node[corridor]
            (l3n2) [right = 0cm of l3n1] { };
        \node[room, thick, red!70!black]
            (l3n3) [right = 0cm of l3n2] {$R$};
        \node[corridor]
            (l3n4) [right = 0cm of l3n3] { };
        \node[room, thick]
            (l3n5) [right = 0cm of l3n4] {$S$};
        \node[corridor]
            (l3n6) [right = 0cm of l3n5] { };
        \node[room, thick, blue!70!black]
            (l3n7) [right = 0cm of l3n6] {$L$};
        %
        \node[coordinate]
            (l4n0) [below = 0cm of l3n0] {$1$};
        \node[corridor]
            (l4n1) [right = 0cm of l4n0] { };
        \node[none]
            (l4n2) [right = 0cm of l4n1] { };
        \node[corridor]
            (l4n3) [right = 0cm of l4n2] { };
        \node[none]
            (l4n4) [right = 0cm of l4n3] { };
        \node[corridor]
            (l4n5) [right = 0cm of l4n4] { };
        \node[none]
            (l4n6) [right = 0cm of l4n5] { };
        \node[corridor]
            (l4n7) [right = 0cm of l4n6] { };
        %
        \node[coordinate]
            (l5n0) [below = 0cm of l4n0] {$2$};
        \node[empty_room]
            (l5n1) [right = 0cm of l5n0] { };
        \node[corridor]
            (l5n2) [right = 0cm of l5n1] { };
        \node[room, thick, blue!70!black]
            (l5n3) [right = 0cm of l5n2] {$L$};
        \node[corridor]
            (l5n4) [right = 0cm of l5n3] { };
        \node[room, thick, yellow!70!black]
            (l5n5) [right = 0cm of l5n4] {$D$};
        \node[corridor]
            (l5n6) [right = 0cm of l5n5] { };
        \node[room]
            (l5n7) [right = 0cm of l5n6] {$R_2$};
        %
        \node[coordinate]
            (l6n0) [below = 0cm of l5n0] {$3$};
        \node[corridor]
            (l6n1) [right = 0cm of l6n0] { };
        \node[none]
            (l6n2) [right = 0cm of l6n1] { };
        \node[corridor]
            (l6n3) [right = 0cm of l6n2] { };
        \node[none]
            (l6n4) [right = 0cm of l6n3] { };
        \node[corridor]
            (l6n5) [right = 0cm of l6n4] { };
        \node[none]
            (l6n6) [right = 0cm of l6n5] { };
        \node[corridor]
            (l6n7) [right = 0cm of l6n6] { };
        %
        \node[coordinate]
            (l7n0) [below = 0cm of l6n0] {$4$};
        \node[empty_room]
            (l7n1) [right = 0cm of l7n0] { };
        \node[corridor]
            (l7n2) [right = 0cm of l7n1] { };
        \node[room]
            (l7n3) [right = 0cm of l7n2] {$R$};
        \node[corridor]
            (l7n4) [right = 0cm of l7n3] { };
        \node[room]
            (l7n5) [right = 0cm of l7n4] {$D$};
        \node[corridor]
            (l7n6) [right = 0cm of l7n5] { };
        \node[empty_room]
            (l7n7) [right = 0cm of l7n6] { };
        %
        \node[coordinate]
            (l8n0) [below = 0cm of l7n0] {$5$};
        \node[corridor]
            (l8n1) [right = 0cm of l8n0] { };
        \node[none]
            (l8n2) [right = 0cm of l8n1] { };
        \node[corridor]
            (l8n3) [right = 0cm of l8n2] { };
        \node[none]
            (l8n4) [right = 0cm of l8n3] { };
        \node[corridor]
            (l8n5) [right = 0cm of l8n4] { };
        \node[none]
            (l8n6) [right = 0cm of l8n5] { };
        \node[corridor]
            (l8n7) [right = 0cm of l8n6] { };
        %
        \node[coordinate]
            (l9n0) [below = 0cm of l8n0] {$6$};
        \node[empty_room]
            (l9n1) [right = 0cm of l9n0] { };
        \node[corridor]
            (l9n2) [right = 0cm of l9n1] { };
        \node[room]
            (l9n3) [right = 0cm of l9n2] {$L$};
        \node[corridor]
            (l9n4) [right = 0cm of l9n3] { };
        \node[empty_room]
            (l9n5) [right = 0cm of l9n4] { };
        \node[corridor]
            (l9n6) [right = 0cm of l9n5] { };
        \node[empty_room]
            (l9n7) [right = 0cm of l9n6] { };
        
        % Corridors
        \path[draw, ultra thick] (l3n5) -- (l3n3);
        \path[draw, ultra thick] (l3n3) -- (l5n3);
        \path[draw, ultra thick] (l3n3) -- (l3n1);
        \path[draw, ultra thick] (l3n3) -- (l1n3);
        
        \path[draw, ultra thick] (l3n5) -- (l3n7);
        \path[draw, ultra thick] (l3n7) -- (l5n7)
            node[pos=0.5,fill=white,inner sep=2]{1};
        
        \path[draw, ultra thick] (l3n5) -- (l5n5);
        \path[draw, ultra thick] (l5n5) -- (l7n5);
        \path[draw, ultra thick] (l7n5) -- (l7n3);
        \path[draw, ultra thick] (l7n3) -- (l9n3)
            node[pos=0.5,fill=white,inner sep=2]{2};

        
        % Wind rose
        \node[draw, circle, semithick, white!50!black, minimum size=2cm] (wind_rose) [right = 1cm of l5n7] {};
        \node[draw, circle, ultra thick, white!50!black, minimum size=1cm] (wr1) at (wind_rose.center) {};
        \node[draw, circle, semithick, white!50!black, minimum size=1.25cm] (wr2) at (wind_rose.center) {};
        % East
        \fill[black] (wind_rose.center) -- ++(0.15, 0.15) -- ++(0.75, -0.15);
        \fill[blue!70!black] (wind_rose.center) -- ++(0.15, -0.15) -- ++(0.75, 0.15);
        % South
        \fill[black] (wind_rose.center) -- ++(0.15, -0.15) -- ++(-0.15, -0.75);
        \fill[yellow!70!black] (wind_rose.center) -- ++(-0.15, -0.15) -- ++(0.15, -0.75);
        % West
        \fill[black] (wind_rose.center) -- ++(-0.15, -0.15) -- ++(-0.75, 0.15);
        \fill[red!70!black] (wind_rose.center) -- ++(-0.15, 0.15) -- ++(-0.75, -0.15);
        % North
        \fill[black] (wind_rose.center) -- ++(-0.15, 0.15) -- ++(0.15, 0.75);
        \fill[white!70!black] (wind_rose.center) -- ++(0.15, 0.15) -- ++(-0.15, 0.75);
        
        %
        \node (N) [above = 0.85cm of wind_rose.center] {N};
        \node (W) [left = 0.85cm of wind_rose.center] {W};
        \node (S) [below = 0.85cm of wind_rose.center] {S};
        \node (E) [right = 0.85cm of wind_rose.center] {E};
        \end{tikzpicture}
        \subcaption{Dungeon level phenotype.}
        \label{fig:grid-translation}
    \end{subfigure}
    
    \caption{Handcrafted example of a genotype-phenotype level translation. (a) presents the level genotype and (b) presents the resulting phenotype. The root node $\boldsymbol{S}$ represents the starting room. Nodes with $\boldsymbol{R}$ (Right), $\boldsymbol{D}$ (Down), and $\boldsymbol{L}$ (Left) represent the direction the parent node connects with them. The numbers in the nodes are keys. The numbers in the dashed edges are the locks. Rooms are always placed in even values of the x and y coordinates, while corridors are placed in coordinates with different parities. By comparing the node colors with the wind rose, we see that a parent room is always considered in the north direction regarding any of its child rooms.}
    \label{fig:tree-representation}
\end{figure}

==> Breno FDG2022/images/results/error.tex <==
\begin{figure}[!t]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            xlabel = Generations,
            ylabel = Fitness,
            height=5cm,
            width=7.5cm,
            scale only axis,
            xmin = -10,
            xmax = 620,
            ymin = -0.5,
            ymax = 7,
            ytick pos=left,
            ytick={0,1,2,3,4,5,6,7},
            xtick={0,100,200,300,400,500,600},
        ]
        % 
        \addplot[clip marker paths=true, color=blue!70!black, mark=none] table [x index=0, y index=1] {images/results/error/data.dat};
        \addplot[blue!70!black, error bars/.cd, y dir=plus, y explicit] table [x index=0, y index=1, y error index=2]{images/results/error/data.dat};
        \addplot[blue!70!black, error bars/.cd, y dir=minus, y explicit] table [x index=0, y index=1, y error index=2] {images/results/error/data.dat}; \label{plot:best}
        % 
        \addplot[clip marker paths=true, color=green!70!black, mark=none] table [x index=0, y index=3] {images/results/error/data.dat};
        \addplot[green!70!black, error bars/.cd, y dir=plus, y explicit] table [x index=0, y index=3, y error index=4]{images/results/error/data.dat};
        \addplot[green!70!black, error bars/.cd, y dir=minus, y explicit] table [x index=0, y index=3, y error index=4] {images/results/error/data.dat}; \label{plot:average}
        % 
        \addplot[clip marker paths=true, color=red!70!black, mark=none] table [x index=0, y index=5] {images/results/error/data.dat};
        \addplot[red!70!black, error bars/.cd, y dir=plus, y explicit] table [x index=0, y index=5, y error index=6]{images/results/error/data.dat};
        \addplot[red!70!black, error bars/.cd, y dir=minus, y explicit] table [x index=0, y index=5, y error index=6] {images/results/error/data.dat}; \label{plot:worst}
        
        \coordinate (legend) at (axis description cs:0.97,0.97);
        \end{axis}
        
        \matrix [
            draw,
            matrix of nodes,
            anchor=north east,
        ] at (legend) {
            \ref{plot:best} & Best Fitness \\
            \ref{plot:average} & Average Fitness \\
            \ref{plot:worst} & Worst Fitness \\
        };
    \end{tikzpicture}

    \caption{Average fitness and standard error of the best, worst and average of elites for each generation, averaged from 100 executions.}
    \label{fig:fitnessEvolution}
\end{figure}

==> Breno FDG2022/images/results/exploration_feedback.tex <==
\begin{figure*}[ht]
    \centering
    
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=3.2cm,
            width=4.5cm,
            ymin = 0,
            ymax = 25,
            ytick={0,5,10,15,20,25},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,3)
            (2,4)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,9)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,19)
            (5,21)
        };
        \end{axis}
    \end{tikzpicture}
    \subcaption{E1.}
    \label{fig:fe_e1}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=3.2cm,
            width=4.5cm,
            ymin = 0,
            ymax = 25,
            ytick={0,5,10,15,20,25},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,2)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,1)
            (5,5)
        };
        \end{axis}
    \end{tikzpicture}
    \subcaption{E2.}
    \label{fig:fe_e2}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=3.2cm,
            width=4.5cm,
            ymin = 0,
            ymax = 25,
            ytick={0,5,10,15,20,25},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,1)
            (2,0)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,2)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,5)
            (5,6)
        };
        \end{axis}
    \end{tikzpicture}
    \subcaption{E3.}
    \label{fig:fe_e3}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=3.2cm,
            width=4.5cm,
            ymin = 0,
            ymax = 25,
            ytick={0,5,10,15,20,25},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,1)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,2)
            (5,6)
        };
        \end{axis}
    \end{tikzpicture}
    \subcaption{E4.}
    \label{fig:fe_e4}
    \end{subfigure}
    
    \caption{Bar charts of answers for question Q5 (``I liked the challenge of finding the keys to this level'') of 57 players for 93 levels. These players answered, through a pre-questionnaire, they enjoy exploring. Each bar corresponds to the number of levels evaluated for the respective value of the five-point Likert scale. Each figure correspond to a descriptors for values of exploration coefficient: E1 = (0.5,0.6), E2 = (0.6,0.7), E3 = (0.7,0.8), E4 = (0.8,0.9), E5 = (0.9,1.0).}
    \label{fig:feedback_exp}
\end{figure*}

==> Breno FDG2022/images/results/feedback.tex <==
\begin{figure*}[ht]
    \centering
    
    \begin{subfigure}[t]{.23\textwidth}
    \centering
        \begin{tikzpicture}[every node/.style={scale=0.8}]
        \tikzstyle{node} = [minimum width=1.6cm, fill=gray!35!white]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=3.75cm,
            width=4.5cm,
            ymin = 0,
            ymax = 55,
            ytick={0,10,20,30,40,50},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,2)
            (2,18)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,21)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,34)
            (5,46)
        };
        \end{axis}
        \node[node] at (0.7,2) {\textbf{AVG: 3.85}};
        \node[node] at (0.7,1.75) {\textbf{STD: 1.13}};
    \end{tikzpicture}
    \subcaption{Q1 - Was it fun?}
    \label{fig:q1}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \tikzstyle{node} = [minimum width=1.6cm, fill=gray!35!white]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=3.75cm,
            width=4.5cm,
            ymin = 0,
            ymax = 55,
            ytick={0,10,20,30,40,50},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,22)
            (2,19)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,32)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,26)
            (5,22)
        };
        \end{axis}
        \node[node] at (0.7,2) {\textbf{AVG: 3.05}};
        \node[node] at (0.7,1.75) {\textbf{STD: 1.35}};
    \end{tikzpicture}
    \subcaption{Q2 - Was it Difficult?}
    \label{fig:q2}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \tikzstyle{node} = [minimum width=1.6cm, fill=gray!35!white]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=3.75cm,
            width=4.5cm,
            ymin = 0,
            ymax = 55,
            ytick={0,10,20,30,40,50},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,15)
            (2,22)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,23)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,38)
            (5,23)
        };
        \end{axis}
        \node[node] at (0.7,2) {\textbf{AVG: 3.26}};
        \node[node] at (0.7,1.75) {\textbf{STD: 1.30}};
    \end{tikzpicture}
    \subcaption{Q3 - Challenge was right?}
    \label{fig:q3}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \tikzstyle{node} = [minimum width=1.6cm, fill=gray!35!white]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=3.75cm,
            width=4.5cm,
            ymin = 0,
            ymax = 55,
            ytick={0,10,20,30,40,50},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,5)
            (2,11)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,23)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,38)
            (5,44)
        };
        \end{axis}
        \node[node] at (0.7,2) {\textbf{AVG: 3.86}};
        \node[node] at (0.7,1.75) {\textbf{STD: 1.13}};
    \end{tikzpicture}
    \subcaption{Q4 - Liked the exploration?}
    \label{fig:q4}
    \end{subfigure}
    
    
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \tikzstyle{node} = [minimum width=1.6cm, fill=gray!35!white]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=3.75cm,
            width=4.5cm,
            ymin = 0,
            ymax = 55,
            ytick={0,10,20,30,40,50},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,7)
            (2,16)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,32)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,28)
            (5,38)
        };
        \end{axis}
        \node[node] at (0.7,2) {\textbf{AVG: 3.61}};
        \node[node] at (0.7,1.75) {\textbf{STD: 1.22}};
    \end{tikzpicture}
    \subcaption{Q5 - Liked finding Keys?}
    \label{fig:q5}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \tikzstyle{node} = [minimum width=1.6cm, fill=gray!35!white]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=3.75cm,
            width=4.5cm,
            ymin = 0,
            ymax = 55,
            ytick={0,10,20,30,40,50},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,31)
            (2,28)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,27)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,13)
            (5,22)
        };
        \end{axis}
        \node[node] at (0.7,2) {\textbf{AVG: 2.72}};
        \node[node] at (0.7,1.75) {\textbf{STD: 1.42}};
    \end{tikzpicture}
    \subcaption{Q6 - Difficult to find exit?}
    \label{fig:q6}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \tikzstyle{node} = [minimum width=1.6cm, fill=gray!35!white]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=3.75cm,
            width=4.5cm,
            ymin = 0,
            ymax = 55,
            ytick={0,10,20,30,40,50},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,17)
            (2,29)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,33)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,18)
            (5,24)
        };
        \end{axis}
        \node[node] at (0.7,2) {\textbf{AVG: 3.02}};
        \node[node] at (0.7,1.75) {\textbf{STD: 1.32}};
    \end{tikzpicture}
    \subcaption{Q7 - Was created by humans?}
    \label{fig:q7}
    \end{subfigure}
    % ~
    % \begin{subfigure}[!t]{.23\textwidth}
    % \centering
    % \scriptsize
    % \vspace{-1.8cm}
    
    % % Tabela completa
    % % \resizebox{\textwidth}{!}{
    % % \begin{tabular}{cccccccc}
    % % \toprule
    % %     & \textbf{Q1} & \textbf{Q2} & \textbf{Q3} & \textbf{Q4} & \textbf{Q5} & \textbf{Q6} & \textbf{Q7} \\
    % % \midrule
    % % \textbf{AVG} & 3.85 & 3.05 & 3.26 & 3.86 & 3.61 & 2.72 & 3.02 \\
    % % \textbf{SD}  & 1.13 & 1.35 & 1.30 & 1.13 & 1.22 & 1.42 & 1.32 \\
    % % \bottomrule
    % % \end{tabular}}
    
    % \begin{tabular}{ccccc}
    % \toprule
    %     & \textbf{Q1} & \textbf{Q2} & \textbf{Q3} & \textbf{Q4} \\
    % \midrule
    % \textbf{AVG} & 3.85 & 3.05 & 3.26 & 3.86 \\
    % \textbf{SD}  & 1.13 & 1.35 & 1.30 & 1.13 \\
    % \bottomrule
    % \end{tabular}
    
    % \vspace{0.2cm}
    
    % \begin{tabular}{cccc}
    % \toprule
    %     & \textbf{Q5} & \textbf{Q6} & \textbf{Q7} \\
    % \midrule
    % \textbf{AVG} & 3.61 & 2.72 & 3.02 \\
    % \textbf{SD}  & 1.22 & 1.42 & 1.32 \\
    % \bottomrule
    % \end{tabular}
    
    % \vspace{0.1cm}
    
    % \subcaption{AVG and SD.}
    % \label{fig:avgsd}
    % \end{subfigure}
    
    \caption{Bar charts of answers of the 74 players for 121 levels. Each bar corresponds to the number of levels evaluated for the respective value of the five-point Likert scale. The questions from \autoref{subsec:feedback} were shortened for brevity.}
    \label{fig:feedback}
\end{figure*}

==> Breno FDG2022/images/results/leniency_feedback.tex <==
\begin{figure*}[ht]
    \centering
    
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=2.8cm,
            width=4.5cm,
            ymin = 0,
            ymax = 14,
            ytick={0,5,10},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,1)
            (2,3)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,4)
            (5,0)
        };
        \end{axis}
    \end{tikzpicture}
    \subcaption{L1.}
    \label{fig:fe_l1}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=2.8cm,
            width=4.5cm,
            ymin = 0,
            ymax = 14,
            ytick={0,5,10},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,1)
            (2,1)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,1)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,3)
            (5,0)
        };
        \end{axis}
    \end{tikzpicture}
    \subcaption{L2.}
    \label{fig:fe_l2}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=2.8cm,
            width=4.5cm,
            ymin = 0,
            ymax = 14,
            ytick={0,5,10},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,3)
            (2,4)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,7)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,4)
            (5,5)
        };
        \end{axis}
    \end{tikzpicture}
    \subcaption{L3.}
    \label{fig:fe_l3}
    \end{subfigure}
    
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=2.8cm,
            width=4.5cm,
            ymin = 0,
            ymax = 14,
            ytick={0,5,10},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,4)
            (2,3)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,5)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,10)
            (5,6)
        };
        \end{axis}
    \end{tikzpicture}
    \subcaption{L4.}
    \label{fig:fe_l4}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.23\textwidth}
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.8}]
        \begin{axis}
        [
            ylabel = Answers,
            xlabel = 5-point Likert Scale,
            ybar stacked,
            height=2.8cm,
            width=4.5cm,
            ymin = 0,
            ymax = 14,
            ytick={0,5,10},
            xtick={1,2,3,4,5},
            every axis plot/.append style={fill},
            nodes near coords={},
        ]
        \addplot [
            red!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,2)
            (2,2)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            blue!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,0)
            (5,0)
        };
        \addplot [
            green!55!white!75!black,
            text=black,
            show sum on top,
        ] coordinates {
            (1,0)
            (2,0)
            (3,0)
            (4,4)
            (5,1)
        };
        \end{axis}
    \end{tikzpicture}
    \subcaption{L5.}
    \label{fig:fe_l5}
    \end{subfigure}
    
    \caption{Bar charts of answers for question Q3 (``The challenge was just right'') of 43 players for 74 levels. These players answered, through a pre-questionnaire, they enjoy battles. Each bar corresponds to the number of levels evaluated for the respective value of the five-point Likert scale. Each figure correspond to a descriptor for leniency values: L1 = (0.5,0.6), L2 = (0.4,0.5), L3 = (0.3,0.4), L4 = (0.2,0.3), L5 = (0.1,0.2).}
    \label{fig:feedback_len}
\end{figure*}

==> Breno FDG2022/images/results/mapelites.tex <==
\begin{figure*}[ht]
    \centering
    
    \begin{tikzpicture}
    
    \node (l1e1) at (0,0) {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l1e1.png}
    };
    \node (l1e2) [right = 0cm of l1e1] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l1e2.png}
    };
    \node (l1e3) [right = 0cm of l1e2] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l1e3.png}
    };
    \node (l1e4) [right = 0cm of l1e3] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l1e4.png}
    };
    \node (l1e5) [right = 0cm of l1e4] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l1e5.png}
    };
    % 
    \node (l2e1) [below = 0cm of l1e1] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l2e1.png}
    };
    \node (l2e2) [right = 0cm of l2e1] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l2e2.png}
    };
    \node (l2e3) [right = 0cm of l2e2] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l2e3.png}
    };
    \node (l2e4) [right = 0cm of l2e3] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l2e4.png}
    };
    \node (l2e5) [right = 0cm of l2e4] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l2e5.png}
    };
    % 
    \node (l3e1) [below = 0cm of l2e1] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l3e1.png}
    };
    \node (l3e2) [right = 0cm of l3e1] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l3e2.png}
    };
    \node (l3e3) [right = 0cm of l3e2] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l3e3.png}
    };
    \node (l3e4) [right = 0cm of l3e3] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l3e4.png}
    };
    \node (l3e5) [right = 0cm of l3e4] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l3e5.png}
    };
    % 
    \node (l4e1) [below = 0cm of l3e1] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l4e1.png}
    };
    \node (l4e2) [right = 0cm of l4e1] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l4e2.png}
    };
    \node (l4e3) [right = 0cm of l4e2] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l4e3.png}
    };
    \node (l4e4) [right = 0cm of l4e3] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l4e4.png}
    };
    \node (l4e5) [right = 0cm of l4e4] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l4e5.png}
    };
    % 
    \node (l5e1) [below = 0cm of l4e1] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l5e1.png}
    };
    \node (l5e2) [right = 0cm of l5e1] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l5e2.png}
    };
    \node (l5e3) [right = 0cm of l5e2] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l5e3.png}
    };
    \node (l5e4) [right = 0cm of l5e3] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l5e4.png}
    };
    \node (l5e5) [right = 0cm of l5e4] {
        \includegraphics[width=.14\textwidth]{images/results/mapelites/l5e5.png}
    };
    
    % Axis
    \node (me1) [below=0cm of l5e1] {E1 (0.5,0.6)};
    \node (me2) [below=0cm of l5e2] {E2 (0.6,0.7)};
    \node (me3) [below=0cm of l5e3] {E3 (0.7,0.8)};
    \node (me4) [below=0cm of l5e4] {E4 (0.8,0.9)};
    \node (me5) [below=0cm of l5e5] {E5 (0.9,1.0)};
    % 
    \node (l1) [below=0cm of me3] {\textbf{Exploration Coefficient}};
    
    \node (ml1) [left=0cm of l1e1] {L1 (0.5,0.6)};
    \node (ml2) [left=0cm of l2e1] {L2 (0.4,0.5)};
    \node (ml3) [left=0cm of l3e1] {L3 (0.3,0.4)};
    \node (ml4) [left=0cm of l4e1] {L4 (0.2,0.3)};
    \node (ml5) [left=0cm of l5e1] {L5 (0.1,0.2)};
    % 
    \node (l2) [rotate=90, above left=0.58cm and 0cm of ml3] {\textbf{Leniency}};
    
    \end{tikzpicture}
    
    \caption{Example of a MAP-Elites population of levels with 20 rooms, 4 keys, 4 locks, 30 enemies, and linear coefficient equal to 2. Each table cell corresponds to an Elite. Descriptors for leniency values: L1 = (0.5,0.6), L2 = (0.4,0.5), L3 = (0.3,0.4), L4 = (0.2,0.3), L5 = (0.1,0.2). Descriptors for values of exploration coefficient: E1 = (0.5,0.6), E2 = (0.6,0.7), E3 = (0.7,0.8), E4 = (0.8,0.9), E5 = (0.9,1.0). The small squares represent corridors, and the bigger squares represent rooms. The white room with a purple square within it is the start room. The purple room with a white square within it is the goal room. White rooms have no enemies while red rooms have enemies within, the more intense the shade of red, the more enemies there are. Colored corridors are locked, and their keys are colored circles within rooms.}
    \label{fig:map-elite-result}
\end{figure*}

==> Breno FDG2022/preamble.tex <==
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{hyperref}

\usepackage{bm}

\usepackage{tikz}
\usetikzlibrary{positioning}
\usetikzlibrary{matrix}

\usepackage{pgfplots, pgfplotstable}
\pgfplotsset{compat=newest}

\pgfplotsset{
    show sum on top/.style={
        /pgfplots/scatter/@post marker code/.append code={%
            \node[
                at={(normalized axis cs:%
                        \pgfkeysvalueof{/data point/x},%
                        \pgfkeysvalueof{/data point/y})%
                },
                anchor=south,
            ]
            {\pgfmathprintnumber{\pgfkeysvalueof{/data point/y}}};
        },
    },
}

\renewcommand{\sectionautorefname}{\uppercase{S}ection}
\renewcommand{\subsectionautorefname}{\uppercase{S}ection}
\renewcommand{\figureautorefname}{\uppercase{F}igure}
\newcommand{\algorithmautorefname}{\uppercase{A}lgorithm}

==> Breno FDG2022/tables/fitness-tables.tex <==
\begin{table*}[ht]
    \centering
    \caption{Results of fitness obtained after 30 executions of our approach. Each table caption represents a set of parameters: (number of rooms)-(number of keys)-(number of locks)-(number of enemies)-(linear coefficient). Each table cell corresponds to an Elite. Descriptors for leniency values: L1 = (0.5,0.6), L2 = (0.4,0.5), L3 = (0.3,0.4), L4 = (0.2,0.3), L5 = (0.1,0.2). Descriptors for values of exploration coefficient: E1 = (0.5,0.6), E2 = (0.6,0.7), E3 = (0.7,0.8), E4 = (0.8,0.9), E5 = (0.9,1.0).}
    \label{tab:fitness_tables}
    
    \begin{subtable}[t]{.5\textwidth}
    \centering
    \caption{15-3-2-20-2.}
    \label{tab:sp1}
    \begin{tabular}{cccccc}
    \toprule
   &              E1 &              E2 &              E3 &              E4 &              E5 \\
    \midrule
L1 &   1.02$\pm$0.61 &   0.84$\pm$0.40 &   0.83$\pm$0.40 &   0.85$\pm$0.38 &  1.06$\pm$0.59 \\
L2 &   0.33$\pm$0.47 &   0.25$\pm$0.40 &   0.23$\pm$0.39 &   0.26$\pm$0.38 &  0.49$\pm$0.57 \\
L3 &   0.09$\pm$0.46 &   0.02$\pm$0.40 &   0.00$\pm$0.40 &   0.04$\pm$0.39 &  0.26$\pm$0.57 \\
L4 &  -0.12$\pm$0.46 &  -0.21$\pm$0.39 &  -0.22$\pm$0.39 &  -0.18$\pm$0.39 &  0.03$\pm$0.54 \\
L5 &   0.05$\pm$0.82 &  -0.15$\pm$0.63 &  -0.19$\pm$0.60 &  -0.15$\pm$0.62 &  0.30$\pm$0.93 \\
    \bottomrule
    \end{tabular}
    \end{subtable}
    ~
    \begin{subtable}[t]{.5\textwidth}
    \centering
    \caption{20-4-4-30-1.}
    \label{tab:sp2}
    \begin{tabular}{ccccc}
    \toprule
            E1 &              E2 &              E3 &              E4 &              E5 \\
    \midrule
0.87$\pm$0.38 &   0.83$\pm$0.36 &   0.81$\pm$0.37 &   0.85$\pm$0.44 &   1.01$\pm$0.54 \\
0.28$\pm$0.40 &   0.26$\pm$0.40 &   0.26$\pm$0.40 &   0.27$\pm$0.39 &   0.32$\pm$0.40 \\
-0.15$\pm$0.44 &  -0.15$\pm$0.43 &  -0.15$\pm$0.43 &  -0.14$\pm$0.44 &  -0.09$\pm$0.43 \\
-0.43$\pm$0.48 &  -0.43$\pm$0.48 &  -0.43$\pm$0.48 &  -0.42$\pm$0.48 &  -0.36$\pm$0.47 \\
-0.47$\pm$0.42 &  -0.47$\pm$0.42 &  -0.46$\pm$0.43 &  -0.45$\pm$0.43 &  -0.34$\pm$0.59 \\
    \bottomrule
    \end{tabular}
    \end{subtable}
    
    
    
    \begin{subtable}[t]{.5\textwidth}
    \centering
    \caption{20-4-4-30-2.}
    \label{tab:sp3}
    \begin{tabular}{cccccc}
    \toprule
   &              E1 &              E2 &              E3 &              E4 &              E5 \\
    \midrule
L1 &   1.17$\pm$0.54 &   0.94$\pm$0.26 &   0.96$\pm$0.25 &   1.00$\pm$0.26 &  1.74$\pm$1.36 \\
L2 &   0.42$\pm$0.26 &   0.40$\pm$0.27 &   0.42$\pm$0.26 &   0.44$\pm$0.26 &  0.77$\pm$0.74 \\
L3 &   0.03$\pm$0.25 &   0.04$\pm$0.27 &   0.04$\pm$0.27 &   0.06$\pm$0.26 &  0.38$\pm$0.73 \\
L4 &  -0.23$\pm$0.26 &  -0.23$\pm$0.27 &  -0.22$\pm$0.27 &  -0.19$\pm$0.27 &  0.13$\pm$0.73 \\
L5 &  -0.06$\pm$0.62 &  -0.15$\pm$0.50 &  -0.25$\pm$0.33 &  -0.20$\pm$0.32 &  0.13$\pm$0.71 \\
    \bottomrule
    \end{tabular}
    \end{subtable}
    ~
    \begin{subtable}[t]{.5\textwidth}
    \centering
    \caption{25-8-8-40-2.}
    \label{tab:sp4}
    \begin{tabular}{ccccc}
    \toprule
            E1 &              E2 &              E3 &              E4 &               E5 \\
    \midrule
1.47$\pm$0.58 &   1.23$\pm$0.32 &   1.35$\pm$0.39 &  1.76$\pm$0.88 &  10.79$\pm$7.38 \\
0.71$\pm$0.32 &   0.63$\pm$0.31 &   0.66$\pm$0.31 &  1.07$\pm$0.78 &   5.82$\pm$4.27 \\
0.43$\pm$0.33 &   0.36$\pm$0.31 &   0.39$\pm$0.32 &  0.80$\pm$0.79 &   5.42$\pm$4.19 \\
0.05$\pm$0.34 &  -0.01$\pm$0.33 &   0.02$\pm$0.32 &  0.43$\pm$0.80 &   4.93$\pm$4.19 \\
-0.02$\pm$0.39 &  -0.04$\pm$0.43 &  -0.09$\pm$0.32 &  0.33$\pm$0.81 &   5.12$\pm$4.47 \\
    \bottomrule
    \end{tabular}
    \end{subtable}
    
    
    
    \begin{subtable}[t]{.5\textwidth}
    \centering
    \caption{30-4-4-50-2.}
    \label{tab:sp5}
    \begin{tabular}{cccccc}
    \toprule
   &              E1 &              E2 &              E3 &              E4 &              E5 \\
    \midrule
L1 &   2.41$\pm$2.26 &   1.69$\pm$0.96 &   1.60$\pm$0.86 &   2.04$\pm$1.44 &   5.33$\pm$5.37 \\
L2 &   0.64$\pm$0.38 &   0.53$\pm$0.25 &   0.55$\pm$0.24 &   0.72$\pm$0.35 &   1.49$\pm$1.40 \\
L3 &   0.06$\pm$0.24 &   0.04$\pm$0.23 &   0.06$\pm$0.24 &   0.20$\pm$0.26 &   0.53$\pm$0.81 \\
L4 &  -0.31$\pm$0.25 &  -0.35$\pm$0.22 &  -0.32$\pm$0.21 &  -0.21$\pm$0.26 &  -0.00$\pm$0.52 \\
L5 &  -0.40$\pm$0.31 &  -0.45$\pm$0.26 &  -0.44$\pm$0.24 &  -0.35$\pm$0.27 &   0.20$\pm$1.10 \\
    \bottomrule
    \end{tabular}
    \end{subtable}
    ~
    \begin{subtable}[t]{.5\textwidth}
    \centering
    \caption{30-6-6-50-1.5.}
    \label{tab:sp6}
    \begin{tabular}{ccccc}
    \toprule
                E1 &              E2 &              E3 &              E4 &              E5 \\
    \midrule
1.36$\pm$1.35 &   1.17$\pm$1.15 &   0.88$\pm$0.72 &   1.40$\pm$1.55 &  5.03$\pm$4.83 \\
0.18$\pm$0.44 &   0.08$\pm$0.19 &   0.04$\pm$0.15 &   0.08$\pm$0.14 &  1.82$\pm$2.09 \\
-0.37$\pm$0.16 &  -0.40$\pm$0.16 &  -0.38$\pm$0.16 &  -0.35$\pm$0.14 &  0.68$\pm$1.57 \\
-0.76$\pm$0.13 &  -0.76$\pm$0.15 &  -0.74$\pm$0.15 &  -0.70$\pm$0.15 &  0.24$\pm$1.50 \\
-0.92$\pm$0.13 &  -0.92$\pm$0.15 &  -0.89$\pm$0.13 &  -0.84$\pm$0.21 &  0.60$\pm$1.94 \\
    \bottomrule
    \end{tabular}
    \end{subtable}
\end{table*}
